OpenACC Acceleration of an Agent-Based Biological Simulation Framework

Computational biology has increasingly turned to agent-based modeling to explore complex biological systems. Biological diffusion (diffusion, decay, secretion, and uptake) is a key driver of biological tissues. GPU computing can vastly accelerate the diffusion and decay operators in the partial differential equations used to represent biological transport in an agent-based biological modeling system. In this paper, we utilize OpenACC to accelerate the diffusion portion of PhysiCell, a cross-platform agent-based biosimulation framework. We demonstrate an almost 40x speedup on the state-of-the-art NVIDIA A100 GPU compared to a serial run on AMD's EPYC 7742. We also demonstrate 9x speedup on the 64 core AMD EPYC 7742 multicore platform. By using OpenACC for both the CPUs and the GPUs, we maintain a single source code base, thus creating a portable yet performant solution. With the simulator's most significant computational bottleneck significantly reduced, we can continue cancer simulations over much longer times.

==> related.tex <==

The directive-based programming model, OpenACC, has been widely used in the past several years to migrate large scale applications demonstrating maturity and stability with the compiler implementations of the high level features. Some of the large (including production) applications that uses OpenACC include MPAS~\cite{yang2019accelerating}, ANSYS~\cite{ansys}, Icosahedral non-hydrostatic (ICON)~\cite{sawyer2014towards}, LQCD Monte Carlo~\cite{bonati2018portable}, and VASP~\cite{maintz2018strategies}. % and other miniapplications such as minisweep~\cite{searles2019mpi,vergara2020experiences}
